Robot Autonomy for Surgery

Autonomous surgery involves having surgical tasks performed by a robot operating under its own will, with partial or no human involvement. There are several important advantages of automation in surgery, which include increasing precision of care due to sub-millimeter robot control, real-time utilization of biosignals for interventional care, improvements to surgical efficiency and execution, and computer-aided guidance under various medical imaging and sensing modalities. While these methods may displace some tasks of surgical teams and individual surgeons, they also present new capabilities in interventions that are too difficult or go beyond the skills of a human. In this chapter, we provide an overview of robot autonomy in commercial use and in research, and present some of the challenges faced in developing autonomous surgical robots.

==> check.tex <==
%% Usage: Latex check.tex
%%
%% Utility to test if all the files required for wspc review volume project
%% are available in your present LaTeX path.
%% - ws-rv975x65.cls
%% - rotating.sty
%% - url.sty
%% - makeidx.sty
%% - chapterbib.sty
%% - cite.sty
%% - ws-index.sty

\newif\onerror

\typeout{*}
\typeout{1. Searching for LaTeX2e ... }
\ifx\documentclass\undefined
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* The WS Review Volume class can only be used with LaTeX2e}
 \typeout{*}
 \typeout{* Stopping...}
 \expandafter\stop
\else
 \typeout{   ... ok}
\fi

\def\next#1/#2/#3\next{#1#2}
\typeout{ }
\typeout{2.  Searching for LaTeX2e version ... }
\ifnum\expandafter\next\fmtversion\next<199612 \relax
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* Your LaTeX version is quite outdated, \fmtversion.}
 \typeout{* The WS Review Volume class can only be used with}
 \typeout{* a recent version of LaTeX2e, please upgrade your installation!}
 \typeout{*}
 \expandafter\stop
\else
 \ifnum\expandafter\next\fmtversion\next<199806 \relax
   \typeout{* Warning: }
   \typeout{*}
   \typeout{* Your LaTeX version is outdated, \fmtversion.}
   \typeout{* We believe that it will probably work, but if you encounter}
   \typeout{* problems you will need upgrade your installation.}
   \typeout{*}
   \typein{* Type <return> to continue ...}
   \errortrue
 \else
   \typeout{   ... ok}
 \fi
\fi

\typeout{ }
\typeout{3. Searching for ws-rv975x65.cls ... }
\IfFileExists{ws-rv975x65.cls}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{* ... ws-rv975x65.cls, file not found! }
     \typeout{*}
     \typeout{* Fatal error occurred:}
     \typeout{*}
     \typeout{* The ws-rv975x65 class file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{4. Searching for graphicx.sty ... }
\IfFileExists{graphicx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... graphicx.sty, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The graphicx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* includegraphics command.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "graphicx".}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{5. Searching for rotating.sty ... }
\IfFileExists{rotating.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... rotating.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The rotating package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* sidewaysfigure and sidewaystable environments.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "rotating".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{6. Searching for url.sty ... }
\IfFileExists{url.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... url.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The url package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use the \string\url}
     \typeout{* command. Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "url".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{7. Searching for makeidx.sty ... }
\IfFileExists{makeidx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... makeidx.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The makeidx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate index.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "makeidx".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{8. Searching for chapterbib.sty ... }
\IfFileExists{chapterbib.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... chapterbib.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The chapterbib package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to include separate bibliography for each chapter.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "chapterbib".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{9. Searching for cite.sty ... }
\IfFileExists{cite.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... cite.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The cite package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate citations in superscript.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "cite".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{10. Searching for ws-rv-har.bst ... }
\IfFileExists{ws-rv-har.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-rv-har.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-rv-har bibliography style file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv975x65 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{11. Searching for ws-rv-van.bst ... }
\IfFileExists{ws-rv-van.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-rv-van.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-rv-van bibliography style file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv975x65 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{12. Searching for ws-index.sty ... }
\IfFileExists{ws-index.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-index.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The ws-index package which is part of the WS RV distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv975x65 class without this package but }
     \typeout{* you can not use multiple indexes.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }

\typeout{13. Searching for ws-rv-thm.sty ... }
\IfFileExists{ws-rv-thm.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... ws-rv-thm.sty, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The ws-rv-thm style file which is part of the WS Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the ws-rv975x65 class without this package but }
     \typeout{* your theorems might render differently.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{* Finished Testing *}
\typeout{ }
\onerror
\typeout{* Some of the files/packages required by WS was not found,}
\typeout{*}
\typeout{* Please review the above comments carefully and update your system.}
\typeout{*}
\typeout{*****************************************************************}
\typein{* Type <return> to continue ...} \else
\typeout{******************************************************}
\typeout{*}
\typeout{* All the files and packages required by WS was found,}
\typeout{* you may now proceed LaTeXing your files.}
\typeout{*}
\typeout{******************************************************} \fi
\stop
\endinput

